DoubleFree:Exploiting Exploration History for Rollout-Free Multi-Task LLMs Training

Multi-task post-training can develop domain specialists through independent reinforcement learning (RL) and consolidate their capabilities through multi-teacher on-policy distillation (MOPD). However, standard MOPD generates on-policy student responses and keeps multiple teachers online throughout consolidation, introducing substantial system costs. We view this pipeline as domain-wise exploration followed by cross-domain exploitation. Domain RL produces not only the final specialists, but also the trajectories collected throughout their training. Existing methods primarily use the former while leaving the latter underutilized. We introduce DoubleFree, which reuses these historical trajectories for rollout-free consolidation and precomputes teacher supervision for online-teacher-free student training. To understand why this works, we analyze when updates from historical trajectories can approximate on-policy distillation updates and how combining trajectories across exploration stages can better support an evolving student. DoubleFree requires only minimal changes to existing post-training frameworks. Across math, code, and instruction following on Qwen3-4B, Qwen3-8B, and SmolLM3-3B, DoubleFree achieves $2.99$-$5.75\times$ consolidation speedups and reduces GPU-hours by $80.9$-$90.1\%$, while maintaining comparable multi-domain performance.

==> Sections/07_statements.tex <==
\section*{AI use statement}
Generative AI tools were used to assist with language polishing and improving the clarity and presentation of the manuscript. All AI-assisted content was reviewed and verified by the authors, who take full responsibility for the content of this paper.

\section*{Ethics statement}
Our work uses publicly available models and benchmarks and involves
no human subjects or personally identifiable information.
The training and evaluation prompts come from established public
datasets cited in Section~\ref{subsec:setup}; we do not introduce new
data collection.
Our method reduces the GPU-hours required for multi-task
consolidation, which lowers the energy footprint of this training
stage; we do not foresee specific negative societal impacts beyond
those generally associated with improved language-model training
efficiency.

\section*{Reproducibility statement}
We describe the explore-exploit formulation and the full \name{}
training procedure in Section~\ref{sec:method}, with the student
objective detailed in Appendix~\ref{app:student_objective}.
Experimental setup, including models, datasets, baselines, training
protocol, and metrics, is given in Section~\ref{subsec:setup} and
Appendix~\ref{app:training_details}.
Proofs of Theorem~\ref{thm:reuse_discrepancy} and
Proposition~\ref{prop:history_coverage} appear in
Appendices~\ref{app:discrepancy_proof} and~\ref{app:coverage_proof}.
All evaluated models, datasets, and benchmarks are publicly available,
and all methods are implemented in the open-source verl
framework~\citep{verl}.
We will release our implementation codes and scripts upon publication.


